Hybrid Contact Preintegration for Visual-Inertial-Contact State Estimation Using Factor Graphs

The factor graph framework is a convenient modeling technique for robotic state estimation where states are represented as nodes, and measurements are modeled as factors. When designing a sensor fusion framework for legged robots, one often has access to visual, inertial, joint encoder, and contact sensors. While visual-inertial odometry has been studied extensively in this framework, the addition of a preintegrated contact factor for legged robots has been only recently proposed. This allowed for integration of encoder and contact measurements into existing factor graphs, however, new nodes had to be added to the graph every time contact was made or broken. In this work, to cope with the problem of switching contact frames, we propose a hybrid contact preintegration theory that allows contact information to be integrated through an arbitrary number of contact switches. The proposed hybrid modeling approach reduces the number of required variables in the nonlinear optimization problem by only requiring new states to be added alongside camera or selected keyframes. This method is evaluated using real experimental data collected from a Cassie-series robot where the trajectory of the robot produced by a motion capture system is used as a proxy for ground truth. The evaluation shows that inclusion of the proposed preintegrated hybrid contact factor alongside visual-inertial navigation systems improves estimation accuracy as well as robustness to vision failure, while its generalization makes it more accessible for legged platforms.

==> Point_Contact.tex <==
\section{Hybrid Point Contact Preintegration}
\label{sec:hybrid_point_contact}

In the case of point contact, the contact orientation is not constrained. Therefore, it is necessary to remove it from the state and optimization framework. We can do this by recognizing that $\C(t) = \R(t) \FK[R](\encoders(t))$ and only using the hybrid preintegration for the contact position. The discrete dynamics now become:
\begin{equation} \label{eq:discrete_point_contact_dynamics}
\begin{aligned}
f &: 
\begin{cases}
	\begin{alignedat}{2}
    \d(t + \Delta t) &= \d(t) - \R(t) \FK[R](\encoders(t)) \noise[][\linearVelocity](t) \Delta t
    \end{alignedat}
\end{cases} \\
\Delta &: 
\begin{cases}
	\begin{alignedat}{2}
    \d[][+] &= \d[][-] + \R \FK[R]^-(\encoders) \FKswitch[p](\encoders)
    \end{alignedat}
\end{cases}
\end{aligned}
\end{equation}
Integrating this hybrid system from time $t_i$ to $t_j$ yields,  
\begin{equation}
\begin{split}
\d[j] = \d[i] &+ \sum_{n=1}^{|\mathcal{S}|} \R[s_n] \FK[R]^-(\encodersM[s_n] - \noise[s_n][\encoders]) \FKswitch[p](\encodersM[s_n] - \noise[s_n][\encoders]) \\
&- \sum_{k=i}^{j-1} \R[k] \FK[R]^-(\encodersM[k] - \noise[k][\encoders]) \noise[k][\linearVelocity] \Delta t  
\end{split}
\end{equation}
We can now rearrange terms to yield a preintegration expression that is independent of the states $\mathcal{X}_i$ and $\mathcal{X}_j$.
\begin{equation}
\begin{split}
\R[i][\transpose](\d[j] - \d[i]) = &\sum_{n=1}^{|\mathcal{S}|} \Delta \R[is_n] \FK[R]^-(\encodersM[s_n] - \noise[s_n][\encoders]) \FKswitch[p](\encodersM[s_n] - \noise[s_n][\encoders]) \\
&- \sum_{k=i}^{j-1} \Delta \R[ik] \FK[R](\encodersM[k] - \noise[k][\encoders]) \noise[k][\linearVelocity] \Delta t 
\end{split}
\end{equation}

\rha{explain why we need to use the noise from imu preintegration}
\begin{equation}
\begin{split}
\Delta \d[ij] &\triangleq \R[i][\transpose](\d[j] - \d[i])\\ 
&= \sum_{n=1}^{|\mathcal{S}|} \Delta \RM[is_n] \Exp(-\delta \anglePhi[is_n]) \Exp\left(\J[\omega][\FK[R]](\encodersM[s_n])\noise[s_n][\encoders]\right) \FK[R](\encodersM[s_n]) \\
& \quad \left( \FKswitch[p](\encodersM[s_n]) - \J[v][\FKswitch[p]](\encodersM[s_n])\noise[s_n][\encoders] \right) \\
& \quad -\sum_{k=i}^{j-1}  \Delta \RM[ik] \Exp(-\delta \anglePhi[ik]) \Exp\left(\J[\omega][\FK[R]](\encodersM[k])\noise[k][\encoders]\right) \FK[R](\encodersM[k]) \noise[k][\linearVelocity] \Delta t 
\end{split}
\end{equation}
After using the first order approximation for the exponential map \eqref{} and removing higher order noise terms, we finally arrive at:
\begin{equation} 
\begin{split}
\Delta \d[ij] \triangleq \R[i][\transpose] (\d[j] - \d[i]) = \Delta \dM[ij] - \delta \d[ij] 
\end{split}
\end{equation}
where $\Delta \dM[ij] \triangleq \sum_{n=1}^{|\mathcal{S}|} \Delta \RM[is_n] \FK[R]^-(\encodersM[s_n]) \FKswitch[p](\encodersM[s_n])$ represents the preintegrated position measurement, and $\delta \d[ij]$ groups all the noise terms together.



==> Visual_Inertial_Factors.tex <==
\section{Visual and Inertial Factors}

\subsection{Visual Odometry}

\subsection{Inertial Odometry}

